ANACONDA: An Improved Dynamic Regret Algorithm for Adaptive Non-Stationary Dueling Bandits

We study the problem of non-stationary dueling bandits and provide the first adaptive dynamic regret algorithm for this problem. The only two existing attempts in this line of work fall short across multiple dimensions, including pessimistic measures of non-stationary complexity and non-adaptive parameter tuning that requires knowledge of the number of preference changes. We develop an elimination-based rescheduling algorithm to overcome these shortcomings and show a near-optimal $\tilde{O}(\sqrt{S^{\texttt{CW}} T})$ dynamic regret bound, where $S^{\texttt{CW}}$ is the number of times the Condorcet winner changes in $T$ rounds. This yields the first near-optimal dynamic regret algorithm for unknown $S^{\texttt{CW}}$. We further study other related notions of non-stationarity for which we also prove near-optimal dynamic regret guarantees under additional assumptions on the underlying preference model.

==> ArXiV/illustration_algo.tex <==
\definecolor{NewGreen}{RGB}{0, 102, 0}
\definecolor{NewBlue}{RGB}{0, 0, 102}
\begin{figure*}[t]
    \centering
   \begin{tikzpicture}[x=50]
      \draw (4, 0.5) node {};

    %     \draw[loosely dotted, thick] (-1,0) -- (-0.7,0);
    %   % first line
    %   \draw (-0.5,0) -- (6.6,0);
      \draw[thick] (-0.2,0) -- (7.4,0);
        
        % second line
      \draw[thick] (8.0,0) -- (8.4,0);
      % first dotted line 
       \draw[loosely dotted, thick] (7.5,0) -- (7.9,0);

      % t_ell
       \draw (-0.2, 0) node[below=7pt] {$t_\ell$};
      \draw[thick] (-0.2,-0.2) -- (-0.2,0.2);
       
       % t_ell+1
       \draw (6.9, 0) node[below=7pt] {$t_{\ell+1}$};       
       \draw[thick] (6.9,-0.2) -- (6.9,0.2);
       
       
        % T
        \draw (8.4, 0) node[below=7pt] {$T$};
      \draw[thick] (8.4,-0.2) -- (8.4,0.2);
       
       % Replay(t_ell, T+1-t_ell)
       \draw (1, 0) node[above=0pt] {$\base(t_\ell, T+1-t_\ell)$};
       
       % Replay(t1, m1)
        \draw (1.4, -1.2) node[above=0pt] {$\base(t_0', m_0')$}; 
       \draw[thick] (0.5, -1.2) -- (2.3, -1.2);
       \draw[thick] (0.5, -1.4) -- (0.5, -1.0);
       \draw[thick] (2.3, -1.4) -- (2.3, -1.0);
       
       % Replay(t2, m2)
       \draw (2.45, -2.4) node[above=0pt] {$\base(t_0'', m_0'')$};
       \draw[thick] (1.2, -2.4) -- (3.5, -2.4);
       \draw[thick] (1.2, -2.6) -- (1.2, -2.2);
       \draw[thick] (3.5, -2.6) -- (3.5, -2.2);
       
        % Replay(t3, m3)
        \draw (5.35, -1.2) node[above=0pt] {$\base(t_0''', m_0''')$}; 
       \draw[thick] (4.6, -1.2) -- (6.1, -1.2);
       \draw[thick] (4.6, -1.4) -- (4.6, -1.0);
       \draw[thick] (6.1, -1.4) -- (6.1, -1.0);
       
       % active 
       \draw[Red, very thick] (-0.2,-0.2) -- (-0.2,0.2);
       \draw[Red, very thick] (-0.2, 0) -- (0.5, 0); 
       
       % firs replay
        \draw[Red, dotted, thick] (0.5,0) -- (0.5,-1);
       \draw[Red, very thick] (0.5,-1.0) -- (0.5,-1.4);
        \draw[Red, very thick] (0.5, -1.2) -- (1.2, -1.2);
        
        % second replay
        \draw[Red, dotted, thick] (1.2,-1.2) -- (1.2,-2.4);
       \draw[Red, very thick] (1.2,-2.2) -- (1.2,-2.6);
        \draw[Red, very thick] (1.2, -2.4) -- (3.5, -2.4);
        \draw[Red, very thick] (3.5,-2.2) -- (3.5,-2.6);
        
        % root replay
        \draw[Red, dotted, thick] (3.5,-0) -- (3.5,-2.4);
        \draw[Red, very thick] (3.5, 0) -- (4.6, 0); 
        \draw[Red, dotted, thick] (4.6,-0) -- (4.6,-1.2);
        \draw[Red, very thick] (6.1, 0) -- (6.9, 0); 
        \draw[Red, very thick] (6.9, 0.2) -- (6.9,-0.2);
        
        % third replay
        \draw[Red, dotted, thick] (6.1,0) -- (6.1,-1);
       \draw[Red, very thick] (4.6,-1.0) -- (4.6,-1.4);
       \draw[Red, very thick] (6.1,-1.0) -- (6.1,-1.4);
        \draw[Red, very thick] (6.1, -1.2) -- (4.6, -1.2);
        
       % restart
        \draw (6.9, 0) node[above=7pt] {{restart}}; 


        %   % t_\ell^a
          \draw (3.1, 0) node[below=7pt] {$t_{\ell}^a$};
        %   \draw (3.2, 0) node[above=7pt] {\small $\mA \backslash \{a\} $ };
          \draw[thick] (3.1,-0.2) -- (3.1,0.2);
           
        % replay arm a
        % \draw [thick, decorate, decoration={brace,amplitude=6pt}, xshift=0pt,yshift=-2pt](4.6,0.4) -- (6.1,0.4) node[midway, yshift=0.5cm] {\footnotesize{$a$ is replayed}};
      \draw (5.35, 0) node[above=0pt] {replay arm $a$};
    %   \draw[thick] (4.6,-0.2) -- (4.6,0.2);
       
       
   \end{tikzpicture}
    \caption{Illustration of the recursive execution of $\base$ within an episode. Any replay can be interrupted by a child replay, whose activity can exceed its parent's lifespan. Here, $t_\ell^a$ denotes the round in episode $\ell$ in which arm $a$ is eliminated from $\mA$. To detect changes in the CW, future calls of $\base$ replay arm $a$.}
    \label{fig:parent_child_replay}
\end{figure*}

==> ArXiV/illustration_proof_sketch.tex <==
\definecolor{NewGreen}{RGB}{0, 102, 0}
\definecolor{NewBlue}{RGB}{0, 0, 102}
\begin{figure}[H]
    \centering
   \begin{tikzpicture}[x=50]
      \draw (0, 0.5) node {};


      \draw[thick] (0,0) -- (4.2,0);
        
         % t_ell
       \draw (0, 0) node[below=7pt] {$t_\ell$};
      \draw[thick] (0,-0.2) -- (0,0.2);
       
       % t_ell+1
       \draw (4.2, 0) node[below=7pt] {$t_{\ell+1}$};       
       \draw[thick] (4.2,-0.2) -- (4.2,0.2);
       
        % tau
       \draw (2.5, 0) node[below=7pt] {$\tau_i$};       
       \draw[thick] (2.5,-0.2) -- (2.5,0.2);
       
        % tau
       \draw (1.5, 0) node[below=7pt] {$t_\ell^{a_{i+1}^*}$};       
       \draw[thick] (1.5, -0.2) -- (1.5, 0.2);
       
       
        % a_i^*
       \draw[thick, ->] (0, 0.7) -- (2.45, 0.7);
        \draw (1.2, 0.8) node[above=1pt] {$a_i^*$ CW};          
        %vertical line
       \draw[thick] (2.5,0.6) -- (2.5,0.8);    
       
       %a_i+1^*
    \draw[thick, ->] (2.5, 0.7) -- (4.15, 0.7);
        \draw (3.3, 0.7) node[above=1pt] {$a_{i+1}^*$ CW};      
        
    \draw (3.3, 0) node[above=1pt] {\tiny detect CW switch by replaying $a_{i+1}^*$};          

   \end{tikzpicture}

\end{figure}

==> ArXiV/limitations.tex <==
\section{Limitations}

\paragraph{Regret Bound.} While our regret bound is optimal in its dependence on $S$ and $T$ (up to logarithmic factors), we expect the linear dependence on $K$ to be suboptimal. The main obstacle in removing this dependence is the importance sampling in \eqref{eq:estimates}, which generally introduces a factor $\sqrt{K(K-1)/2}$ in the context of dueling bandits (see e.g.\ \cite{saha2022versatile}). 

\begin{rem}
    The logarithmic dependence on $T$ in Theorem~\ref{thm:main_result} can be reduced to ... by setting the elimination rule to ... and tightening the concentration bound of Lemma~\ref{prop:concentration_bound} in accordance with Lemma~... to ...  
\end{rem} 

\paragraph{Runtime.} Checking for the elimination rule \eqref{eq:elim} has runtime $O(K^2 t^2)$ in its current form. 


==> ArXiV/macro2.tex <==

\def\QED{{\phantom{x}} \hfill \ensuremath{\rule{1.3ex}{1.3ex}}}
\newcommand{\extraproof}[1]{\rm \trivlist

\item[\hskip \labelsep{\bf Proof of #1. }]}
\def\endextraproof{\QED \endtrivlist}

\newenvironment{rtheorem}[3][]{

\bigskip

\noindent \ifthenelse{\equal{#1}{}}{\bf #2 #3}{\bf #2 #3 (#1)}
\begin{it}
}{\end{it}}

\newcommand{\nonl}{\renewcommand{\nl}{\let\nl}}
\def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}
\newcommand{\obs}{o}

% enable do while
\SetKwRepeat{Do}{do}{while}

